A classification model based on a population of hypergraphs

This paper introduces a novel hypergraph classification algorithm. The use of hypergraphs in this framework has been widely studied. In previous work, hypergraph models are typically constructed using distance or attribute based methods. That is, hyperedges are generated by connecting a set of samples which are within a certain distance or have a common attribute. These methods however, do not often focus on multi-way interactions directly. The algorithm provided in this paper looks to address this problem by constructing hypergraphs which explore multi-way interactions of any order. We also increase the performance and robustness of the algorithm by using a population of hypergraphs. The algorithm is evaluated on two datasets, demonstrating promising performance compared to a generic random forest classification algorithm.

==> Sections/Old_Methods.tex <==
In this section we present the notation and a framework for a supervised learning method to sort grains into species.


analyse the dataset described in Section ??. 

The raw data comprises of  ??? items, where each item corresponds to
\begin{itemize}
    \item an individual grain, termed a {\em point};
    \item recording a measurement for 16 different features.
\end{itemize}
The object is to develop a model that can sort the grains into ??? different species, termed {\em classes.}

Initially the data is stored in an $??? \times 16$ array  labelled $F=[f_{i,j}]$ where, for $i=1,\dots, ???$ and $j=1,\dots, 16$,  $f_{i,j}$ records to the measurement of grain $i$ with respect to feature $j$.

\subsection{Normalising and Discretising Data}

The entries in the array $F$ (raw data) will be normalised and transformed into a standard $z$-score, as described in \eqref{eq:norm_matrix}. Then each score will be  mapped to a bin  or interval as described in 
\eqref{eq:binning}.

Formally, for each column $j$, $j=1,\dots, 16$, of $F$ calculate the mean, denoted $\mu_j$, and the standard deviation  $\sigma_j$. For $\alpha \in \mathbb{R}$ and $\ell \in \mathbb{R}^+$, let $P_{\ell,\alpha}=\{[ (t-1)\ell + \alpha, t\ell + \alpha ), [- t\ell + \alpha, (-t+1)\ell + \alpha )\mid t\in \mathbb{Z}^+\}$ be a partition of the reals,
\begin{equation}\label{eq:reals_intervals_alpha}
   (-\infty,\infty) = \bigcup\limits_{t = 1}^{\infty} \Big[ (t-1)\ell + \alpha, t\ell + \alpha \Big) \ \cup \ \bigcup\limits_{t = -1}^{-\infty} \Big[ t\ell + \alpha, (t+1)\ell + \alpha \Big).
\end{equation}
This partition is parameterised by, the uniform interval length $\ell$ and the central point  $\alpha$ termed the origin.  
Now construct a $???\times 16$ array $S=[s_{i,j}]$ by executing  the following algorithm.

\noindent{\bf Algorithm: Normalising and Binning}
\begin{itemize}  
\item For $i=1,\dots, ??$ and $j=1,\dots, 16$, transform $f_{i,j}$ into the $z$-score given in \eqref{eq:norm_matrix}.
    \begin{equation}\label{eq:norm_matrix}
    z_{i,j} = \frac{f_{i,j} - \mu_j}{\sigma_j}.
\end{equation}
    Note that for fixed $j$, the  mean of $z_{i,j}$ is zero and standard deviation  one.
\item Define a function $s:\mathbb{R}\rightarrow \mathbb{Z}\setminus \{0\}$, where
\begin{equation}\label{eq:binning}
s(z_{i,j})=\left\{
\begin{array}{ll}
t, & \mbox{if }
z_{i,j}\in [ (t-1)\ell + \alpha, t\ell + \alpha )\\
-t, & \mbox{if }
z_{i,j}\in [- t\ell + \alpha, (-t+1)\ell + \alpha ).\end{array}
\end{equation}
\item Let $S=[s_{i,j}]$ be a $??\times 16$ array where $s_{i,j}=s(z_{i,j})$.

\end{itemize}








\subsection{Cross-Validation}




 To evaluate the accuracy and performance of the method, we will implement $5$-fold cross validation, by dividing the dataset into training data and validation data, achieved by  partitioning the matrix $S$ into two submatrices $B = [b_{ij}]$ as the training data matrix and $V = [v_{ij}]$ as the validation data matrix. 

\subsection{Main Effects (Updated Version)}

We recall that $S = [ s_{i,j} ]$ is the discrete data matrix for all points and features. To build a model based on training data, we consider the submatrix $B = [ b_{i,j} ]$, which contains the discrete data for training points only. We also introduce the notation $\{ Q_c \mid c = 1,\dots,7 \}$, where $Q_i$ is the set of training points belonging to class $i$. 

We now look to construct a matrix for each feature, or column of $B$. This matrix will be denoted $\hat{M}_k = [ \hat{m}_{t,c} ]$ for feature $k$. The entries for these matrices are defined in \eqref{eq:M_matrix}.
\begin{equation}\label{eq:M_matrix}
    \hat{m}_{t,c} = \frac{\Big\vert \{ (i,k) \mid i \in Q_c, \ b_{i,k} = t - 1 + \min {t} \} \Big\vert}{\Big\vert Q_c \Big\vert}
\end{equation}
This definition produces a matrix for each feature, where entries correspond to a particular class and interval, giving the proportion of points in the class which satisfy that interval. Therefore the columns sum to one. 

We now normalise each matrix so that the sum of each row is one, generating the row normalised matrix $M_k = [ m_{t,c} ]$ for each feature $k$, defined in \eqref{eq:M_normalised}.
\begin{equation}\label{eq:M_normalised}
    m_{t,c} = \frac{\hat{m}_{t,c}}{\sum\limits_c \hat{m}_{t,c}}
\end{equation}
Since each row sums to one, we consider each row as a distribution for each interval. This allows the model to describe the probability that a particular interval belongs to a class. 

With this, we now have a set of matrices, $\{ M_k \mid k = 1, \dots, 16 \}$, which summaries the discrete information for each feature based on the partition $P_{\ell,\alpha}$.






\subsection{Main Effects}\label{section:main_effects}

To study the main effects, we will generate a population of models based on the training dataset $B$, where each feature is considered individually. We first define a model based on discretisation. \textit{Discretisation} is the process of partitioning continuous features into nominal intervals. That is, we map each point of the training dataset to an integer based on a given partition. In order to define such a model, we must first describe a partition of the real numbers. We will use uniform intervals to partition the real numbers as described by $T$ in \eqref{eq:reals_intervals}, with interval length defined as $\ell$.

 Since we are interested in the main effects, we do this column-wise as to study each feature individually. As such, we generate a matrix, $S_{\phi}$, for each feature $\phi$, which stores the distribution of each class per interval. That is, for column $\phi$ of $S$, denoted $S_{\phi}$, we can count the number of occurrences of $t=\tau$ for each of the $k$ classes, denoted $c^{\phi}_i(\tau)$ for class $i$. These values will make up the entries of $F_{\phi} = [f^{\phi}_{ij}]$, as defined in \eqref{eq:F_matrix}. We note that the function $P$ will output negative integers in some cases, we define $t_{\min}$ as the smallest $t$ value achieved in $S$. Similarly, we define $t_{\max}$ as the largest $t$ achieved in $S$.
\begin{equation}\label{eq:F_matrix}
    f^{\phi}_{ij} = c^{\phi}_j(i + t_{\min}-1), \ i = 1,\dots,t_{\max}+(-t_{\min})+1
\end{equation}
With this definition, we see that columns indicate classes and row $i$ corresponds to the interval $t = i + t_{\min}-1$; such that row $1$ corresponds to interval $t=t_{\min}$. We note here that in some cases the entire row will be zeros, indicating that a particular interval is not satisfied by any of the training points. 

We can now generate a set of matrices $\mathcal{F} = \{ F_{\phi} \mid \phi = 1,\dots,m \}$, where each matrix corresponds to one of the $m$ features under consideration. We normalise these matrices as the entries are counts. We first do this by normalising the columns such that they sum to one, thereby generating the matrix $G_{\phi}=[g^{\phi}_{ij}]$, entries defined in \eqref{eq:G_matrix}.
\begin{equation}\label{eq:G_matrix}
    g^{\phi}_{ij} = \frac{f^{\phi}_{ij}}{ \sum\limits_j f^{\phi}_{ij}}
\end{equation}
From this, we see that the entries of $G_{\phi}$ give the proportion of the class which satisfy each particular interval. However, we desire each row to sum to one, so that we can consider the rows as being a distribution for the respective interval. We then row normalise the matrix $G_{\phi}$ to produce the matrix $\hat{F}_{\phi} = [\hat{f}^{\phi}_{ij}]$, with entries defined in \eqref{eq:F_hat}.
\begin{equation}\label{eq:F_hat}
    \hat{f}^{\phi}_{ij} = \frac{g^{\phi}_{ij}}{\sum\limits_i g^{\phi}_{ij}}
\end{equation}
Therefore, the set of matrices $\hat{\mathcal{F}} = \{ \hat{F}_{\phi} \mid \phi = 1, \dots, m \}$ summarises the main effects via the partition $P$ with parameters $(\ell,\alpha)$. In particular, each matrix represents an individual feature, where rows correspond to particular intervals and columns indicate classes. We note that each row sums to one, thus each row can be considered a distribution of the interval across classes. This set of matrices is considered to be a trained model under the parameters $(\ell,\alpha)$. 

We now evaluate the accuracy of the model using the validation dataset. In order to do this, we first recall the matrix $V = [v_{ij}]$, which contains the $z$-scores for each validation data point (row) and feature (column). We then apply the partition function $P$ as described in \eqref{eq:P_function} with parameters $(\ell,\alpha)$ as in the model. As such, we generate the matrix $W = [w_{ij}]$, with entries defined in \eqref{eq:W_matrix}.
\begin{equation}\label{eq:W_matrix}
    w_{ij} = P(v_{ij})
\end{equation}
This matrix gives the interval $t$ that is satisfied for each validation point and feature. Moreover, each interval $t$ in each column of this matrix corresponds to particular matrix and row of $\hat{\mathcal{F}}$. As such, for each validation point $v$, we construct a matrix, $A_v = [a^v_{ij}]$ which contains the satisfied row of the corresponding matrix of $\hat{\mathcal{F}}$, where the entries are defined in \eqref{eq:A_matrix}.
\begin{equation}\label{eq:A_matrix}
    a^v_{ij} = \hat{f}^i_{w_{vj}+t_{\min}-1,j}
\end{equation}
Therefore the matrix $A_v$ corresponds to validation point $v$, where columns indicate classes and rows give the class distribution (from the model) attained for a particular feature according to the interval satisfied by the validation point. 

To predict a class for each validation point, we reduce each matrix to a tuple. We do this by calculating the average of each column (class). That is, we transform each matrix $A_v$ to a tuple $U_v = [u^v_j]$, as per \eqref{eq:mean_vec}, where $m$ is the number of features.
\begin{equation}\label{eq:mean_vec}
    u^v_j = \frac{\sum\limits_{x=1}^{m} a^v_{xj}}{m}
\end{equation}
This tuple then summarises the information for each class. To predict a class for a validation point, we select the class which achieves the maximum entry among this tuple. This is the prediction attained from the model based on the partition $P$ with parameters $(\ell,\alpha)$.

To generate a population of models, and thus predictions, we vary the parameters $(\ell,\alpha)$. In fact, we can select any number of interval lengths $l$ and explore various origin values, $\alpha$. Specifically, if we consider the set of interval lengths $\bm{\ell} = \{ \ell_1,\dots,\ell_n \}$ and the set of origins $\bm{\alpha} = \{ \alpha_1, \dots, \alpha_m \}$ per length. Then we will be studying $nm$ models; $nm$ class predictions for each validation point. We take the most occurring (mode) class of the $nm$ models as the final prediction for each validation point. 

\subsection{Two-Way Interactions}\label{sec:two_way}

In this section we define the supervised learning method which explores two-way interactions, known as \textit{Bipartite Bins}. We use similar techniques as Section \ref{section:main_effects}, with the caveat that we manipulate these to explore the two-way interactions. 

We now discuss the steps taken to build the model from the training dataset. We begin with the normalised data matrix $B$, which contains the $z$-scores for each data point and feature. Since we are interested in exploring the two-way interactions, we must consider all distinct pairs of features. That is, if there are $m$ features, then there are ${m \choose 2}$ distinct pairs of features. Going forward, we define this set of distinct pairs of features as a set of conditions. We define the set of conditions as $\gamma = \{ (c_{1,1},c_{1,2}), (c_{2,1},c_{2,2}), \dots, (c_{{m \choose 2},1},c_{{m \choose 2},2}) \}$. As such, we now define the matrix $R = [r_{ij}]$, where entries capture the the pairs of interval values for each data point and condition, as per \eqref{eq:2way_datamatrix}.
\begin{equation}\label{eq:2way_datamatrix}
    r_{ij} = (s_{i,c_{j,1}},s_{i,c_{j,2}})
\end{equation}
In this way, the matrix $R$ summarises all two-way interactions between all features per data point. 

We are now interested in finding the proportion of each class which satisfy each pair of intervals. That is, for condition $\phi \in \gamma$, we count the number of occurrences of $(\tau_1,\tau_2)$ for each of class and divide by the size of the class, denoted $c_i^{\phi}(\tau_1,\tau_2)$ for class $i$. We now store this information using a $3$-dimensional tensor, where rows and columns correspond to the first and second entry of the interval pair, while the tubes (third dimension) correspond to the classes. As such, we can generate the tensor $F_{\phi} = [f_{ijk}]$ for condition $\phi$, with entries defined in \eqref{eq:F_tensor}.
\begin{equation}\label{eq:F_tensor}
    f_{ijk} = c^{\phi}_k (i + t_{\min} - 1, j + t_{\min} - 1), \ i = 1,\dots,t_{\max}+(-t_{\min})+1
\end{equation}

We now look to normalise each tube of the tensor $F_{\phi}$. We do this as each tube associates to a unique interval pair and we want each tube to describe a distribution with respect to the classes. As such, we normalise each tube to sum to one, generating a normalised the normalised tensor $\hat{F}_{\phi} = [\hat{f}^{\phi}_{ijk}]$, defined in \eqref{eq:F_tensor_norm}.
\begin{equation}\label{eq:F_tensor_norm}
    \hat{f}^{\phi}_{ijk} = \frac{f_{ijk}}{\sum\limits_k f_{ijk}} = \hat{f}^{\phi} (i,j,k)
\end{equation}
We now have a set of normalised tensors, $\hat{\mathcal{F}} = \{ \hat{F}_{\phi} \mid \phi = 1, \dots, {m \choose 2} \}$, based on the training data. This set of tensors will be the model we use to predict the class of the respective validation dataset. 

We now discuss how we use the described model to predict the class of each validation point. We first recall the matrix $W$ (from \eqref{eq:W_matrix}), which contains the interval number satisfied for each validation point and feature. With this, we generate a new matrix $Q = [q_{ij}]$, with entries defined in \eqref{eq:Q_matrix}.
\begin{equation}\label{eq:Q_matrix}
    q_{ij} = (w_{i,c_{j,1}},w_{i,c_{j,2}})
\end{equation}
The matrix $Q$ then summarises the pairs of intervals satisfied for each validation point (row) and condition (column). We now consider each validation point individually and construct a matrix accordingly, $Y_v = y_{ij}$ for point $v$. The rows of this matrix will correspond to conditions and columns representing classes, as described in \eqref{eq:Y_matrix}.
\begin{equation}\label{eq:Y_matrix}
    y^v_{ij} = \hat{f}^i(w_{v,(c_i,1)} + t_{\min} - 1, w_{v,(c_i,2)} + t_{\min} - 1, j)
\end{equation}

We now have a matrix for each validation point where rows give the distribution over classes for the satisfied interval pair according to the model. To make a prediction we construct the tuple, $Z_v = [z^v_j]$, where each entry defined in \eqref{eq:Z_tuple}, is the column mean of $Y_v$, giving the mean score of each class. 
\begin{equation}\label{eq:Z_tuple}
    z^v_j = \frac{\sum\limits_{x=1}^m y^v_{xj}}{m}
\end{equation}
We then select the class which attains the maximum mean score from $Z_v$ as the predicted class for validation point $v$.

We recall that this model and prediction was made using a particular partition $P$, with parameters $(\ell,\alpha)$. As suggested in Section \ref{section:main_effects}, we can create a population of models with various parameters, producing a population of class predictions per validation point. We again, will take the most occurring (mode) class as the final prediction for a validation point. 

\subsubsection{Results}

To evaluate the performance of the above methods, we look at the $5$-fold cross-validation accuracy across all classes. In Figure \ref{fig:main_effects_results}, we compare the performance to the accuracy of a random forest and also present the accuracy level for each fold.  

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.5\textwidth]{bins.eps}
    \caption{Accuracy results from method and random forest.}
    \label{fig:main_effects_results}
\end{figure}

\subsection{Graphs and Hypergraphs}

In this section, we present a supervised learning method which incorporates graph and hypergraph theory. To generate a model based on training data, we make use of backbones and centrality measures. To evaluate the performance of the model, we then predict the class of each validation point using hypergraphs and centrality measures. 




We begin by defining the raw data matrix. This matrix will contain the unnormalised data for each point (row) and feature (column). We will denote this matrix as $D = [d_{ij}]$, with entries defined in \eqref{eq:raw_matrix}, where $f_{i,j}$ corresponds to the value given to grain $i$ and feature $j$.
\begin{equation}\label{eq:raw_matrix}
    d_{ij} = f_{i,j}
\end{equation}
Since there are $n$ grains and $m$ features, $D$ is $n \times m$. 
